Rethinking Ductility -- A Study Into the Size-Affected Fracture of Polymers

Ductility quantifies a material's capacity for plastic deformation, and it is a key property for preventing fracture driven failure in engineering parts. While some brittle materials exhibit improved ductility at small scales, the processes underlying this phenomenon are not well understood. This work establishes a mechanism for the origin of ductility via an investigation of size-affected fracture processes and polymer degree of conversion (DC) in two-photon lithography (TPL) fabricated materials. Microscale single edge notch bend ($\mu$SENB) specimens were written with widths from 8 to 26 $\mu$m and with different laser powers and post-write thermal annealing to control the DC between 17\% and 80\%. We find that shifting from low to high DC predictably causes a $\sim$3x and $\sim$4x increase in strength and bending stiffness, respectively, but that there is a corresponding $\sim$6x decrease in fracture energy from 180 $J/m^2$ to 30 $J/m^2$. Notably, this reduced fracture energy is accompanied by a ductile-to-brittle transition (DBT) in the failure behavior. Using finite element analysis, we demonstrate that the DBT occurs when the fracture yielding zone size ($r_p$) approaches the sample width, corresponding with a known fracture size-affected transition from flaw-based to strength-based failure. This finding provides a crucial insight that ductility is a size-induced property that occurs when features are reduced below a characteristic fracture length scale and that strength, stiffness, and toughness alone are insufficient predictors of ductility.

==> Section/Abstract.tex <==
Two-photon polymerization direct laser writing (TPP-DLW) is an emergent additive manufacturing technique which enables the creation of parts with nanoscale features, enabling the utilization of enhanced properties of nanomaterials.
This study explores the impact of print parameters on the fracture toughness of structures fabricated using two-photon polymerization direct laser writing (TPP-DLW). 
The variation of laser power, scanning speed, and layer thickness ultimately changes the polymer degree of conversion, and we analyze the impact of DC on the fracture toughness of the printed structures. 
Our results demonstrate that varying the DC can significantly alter the fracture toughness of the printed structures, with significant reduction in toughness with increasing DC.
By means of a systematic Linear elastic fracture mechanics (LEFM) and Size-effect law (SEL) fracture analysis, we further show that the ductile to brittle transition in fracture behavior with increasing DC occurs due to 1 order of magnitude reduction in the process zone size from 100 $\mu$m  to 3 $\mu$m.
% We also show that the incorporation of the heterogeneity principle can improve the fracture toughness of TPP-DLW structures, which is essential for their use in various fields such as microfluidics, tissue engineering, and microelectromechanical systems. 
Our findings provide important insights into the relationship between print parameters and fracture toughness in TPP-DLW structures, which can guide the development of improved printing techniques and materials for advanced applications.
